Error Identification and Recovery in Robotic Snap Assembly

Existing methods for predicting robotic snap joint assembly cannot predict failures before their occurrence. To address this limitation, this paper proposes a method for predicting error states before the occurence of error, thereby enabling timely recovery. Robotic snap joint assembly requires precise positioning; therefore, even a slight offset between parts can lead to assembly failure. To correctly predict error states, we apply functional principal component analysis (fPCA) to 6D force/torque profiles that are terminated before the occurence of an error. The error state is identified by applying a feature vector to a decision tree, wherein the support vector machine (SVM) is employed at each node. If the estimation accuracy is low, we perform additional probing to more correctly identify the error state. Finally, after identifying the error state, a robot performs the error recovery motion based on the identified error state. Through the experimental results of assembling plastic parts with four snap joints, we show that the error states can be correctly estimated and a robot can recover from the identified error state.

==> section/05_results.tex <==
\section{Construction of decision tree}
\label{4.4}
% \ref{4.3}節で抽出された特徴量に対して，アルゴリズム\ref{algorithm_SVM}を用いて決定木を構築した(図\ref{decision tree})．
% また本実験では，
% 一個抜き交差検証(leave-one-out cross-validation)に従い，
% SVMによる分類を行った．
% 以下に，
% スナップ工程において$t_{span}=2.0[\mathrm{s}]$において抽出された特徴量に対して構築された決定木，及び，各ノードにおけるSVMの実行結果を
% 図\ref{decision tree}，図\ref{classifier}に示す．
% また，$t_{span}=1.8[\mathrm{s}]$，$t_{span}=1.9[\mathrm{s}]$，$t_{span}=2.0[\mathrm{s}]$において構築された各ノードでの式\ref{accuracy}に基づく分類精度を
% 表\ref{node accuracy}に示す．
% ここで，
% 図\ref{decision tree}について，
% 各ノードにはSVMが実行された力・トルク成分，及び分類された成否パターン群を示している．
% また図\ref{classifier}(a)$\sim$(h)について，
% 〇と\triangle{}は分類された成否パターン群それぞれに属する特徴量であり，
% ●，▲
% はサポートベクトルである．

\begin{figure}[p]
  \begin{center}
          \includegraphics[width=\linewidth]{picture/chap4/SVM/decision_tree_1stmove.eps}
          \caption{Decision tree about snap process when $t_{span}=2.0[\mathrm{s}]$}
          \label{decision tree}
        \end{center}
\end{figure}

% \begin{figure}[h]
%  \begin{minipage}[b]{0.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_result_1stmove_1stnode_Fz_0~200.eps}
%   \subcaption{Node 1(torque about $y$ axis)}
%  \end{minipage}
%  \begin{minipage}[b]{0.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_result_1stmove_2ndnode_Ty_0~200.eps}
%   \subcaption{Node 2(force in $z$ direction)}
%  \end{minipage}\\
%  \begin{minipage}[b]{0.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_result_1stmove_3rdnode_Ty_0~200.eps}
%   \subcaption{Node 3(force in $y$ direction)}
%  \end{minipage}
%  \begin{minipage}[b]{0.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_result_1stmove_4thnode_Ty_0~200.eps}
%   \subcaption{Node 4(torque about $x$ axis)}
%  \end{minipage}\\
%  \begin{minipage}[b]{0.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_result_1stmove_5thnode_Fz_0~200.eps}
%   \subcaption{Node 5(force in $x$ direction)}
%  \end{minipage}
%  \begin{minipage}[b]{0.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_result_1stmove_6thnode_Tz_0~200.eps}
%   \subcaption{Node 6(torque about $z$ axis)}
%  \end{minipage}\\
%  \begin{minipage}[b]{0.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_result_1stmove_7thnode_Ty_0~200.eps}
%   \subcaption{Node 7(force in $y$ direction)}
%  \end{minipage}
%  \begin{minipage}[b]{0.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_result_1stmove_8thnode_Tz_0~200.eps}
%   \subcaption{Node 8(force in $x$ direction)}
%  \end{minipage}
%  \caption{Results of applying SVM to feature quantities for each node in Fig.\ref{decision tree}}
%      \label{classifier}
% \end{figure}

% \begin{figure}[p]
%   \begin{center}
%     \begin{tabular}{c}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_1stmove_1st_Ty.eps}
%           \hspace{1.6cm} (a)Node 1(torque about $y$ axis)
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_1stmove_2nd_Fz.eps}
%           \hspace{1.6cm} (b)Node 2(force in $z$ direction)
%         \end{center}
%       \end{minipage}
%      \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_1stmove_3rd_Fy.eps}
%           \hspace{1.6cm} (c)Node 3(force in $y$ direction)
%         \end{center}
%       \end{minipage}\\
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_1stmove_4th_Tx.eps}
%           \hspace{1.6cm} (d)Node 4(torque about $x$ axis)
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_1stmove_5th_Fx.eps}
%           \hspace{1.6cm} (e)Node 5(force in $x$ direction)
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_1stmove_6th_Tz.eps}
%           \hspace{1.6cm} (f)Node 6(torque about $z$ axis)
%         \end{center}
%       \end{minipage}\\
%       \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_1stmove_7th_Fy.eps}
%           \hspace{1.6cm} (g)Node 7(force in $y$ direction)
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/SVM/SVM_1stmove_8th_Fx.eps}
%           \hspace{1.6cm} (h)Node 8(force in $x$ direction)
%         \end{center}
%       \end{minipage}
%     \end{tabular}
%     \caption{Results of applying SVM to feature quantities for each node in Fig.\ref{decision tree}}
%     \label{classifier}
%   \end{center}
% \end{figure}

% \begin{center}
% \begin{table}[t]
% \begin{center}
% \caption{Accuracy based on formulate\ref{accuracy} at each node in decision trees of snap process[\%]}
% \scalebox{0.85}{  
% \begin{tabular}{|c|c|c|c|} \hline
%   \multirow{Data span $t_{span}[\mathrm{s}]$} & 1.8 & 1.9 & 2.0 \\ \hline \hline
%     Node1 & ~0.088~ & ~0.044~ & ~0.044~\\ \cline{1-4}
%     Node2 & ~0.039~ & ~0.000~ & ~0.000~\\ \cline{1-4}
%     Node3 & ~0.076~ & ~0.077~ & ~0.077~\\ \cline{1-4}
%     Node4 & ~0.167~ & ~0.063~ & ~0.063~\\ \cline{1-4}
%     Node5 & ~0.000~ & ~0.000~ & ~0.000~\\ \cline{1-4}
%     Node6 & ~0.067~ & ~0.030~ & ~0.030~\\ \cline{1-4}
%     Node7 & ~0.500~ & ~0.000~ & ~0.000~\\ \cline{1-4}
%     Node8 & ~0.500~ & ~0.250~ & ~0.250~\\ \hline
%   \end{tabular}
% }
%   \label{node accuracy}
%   \end{center}
% \end{table}
% \end{center}
% 表\ref{node accuracy}より，
% $t_{span}=1.8[\mathrm{s}]$までの波形データを用いた場合，
% ノード7，8において分類精度が低いことが確認できる．
% 一方，$t_{span}=1.9[\mathrm{s}]$以降の波形データを追加した場合，
% 各ノードにおいて分類精度が高いことが確認できた．
% よって，十分な識別精度を得るために，
% スナップ工程では
% $t_{span}=1.9[\mathrm{s}]$程度までの力情報が重要であり，
% $t_{span}=1.8[\mathrm{s}]$までの早い段階での力情報のみでは作業途中での識別が困難であると考えられる．

\subsection{Identification during assembly}
\label{4.5}
% \ref{4.2}節で取得した検証用の波形データに対して，
% $t_{span}$を$t_{span}=1.8[\mathrm{s}]$，$t_{span}=1.9[\mathrm{s}]$，$t_{span}=2.0[\mathrm{s}]$として，それぞれのデータ区間に対して特徴量を抽出し，\ref{4.4}節で構築された対応するデータ区間における決定木を用いて成否パターンの識別を行うことで，どの程度早い段階で正しい識別が可能であるのかを検証した．
% 検証用のデータとして，
% 表\ref{identify detail}
% に示すように，成否パターン(1)については45回スナップアセンブリを，
% 成否パターン(2)$\sim$(9)については各5回スナップアセンブリを行い，
% 計85回分のスナップ工程，探り動作工程における波形データを取得し，成否パターンの識別を行った．
% 探り動作工程を導入せずにスナップ工程のみで識別を行った結果を
% 表\ref{identify snap process}に，
% スナップ工程での識別結果を用いずに探り動作工程のみで識別を行った結果を
% 表\ref{identify search process}に，
% \ref{3.5}節に従い，探り動作工程を導入した際の識別結果を
% 表\ref{identify both processes}に，
% 成否パターンそれぞれに対する識別結果を
% 表\ref{identify detail}
% に示す．ここで，表\ref{identify detail}では，$t_{span}=2.0[\mathrm{s}]$での識別結果のみを示す．


% \begin{center}
% \begin{table}[!h]
% \begin{center}
% \caption{Result of identification by snap process}
% \scalebox{0.85}{  
% \begin{tabular}{|c|c|c|} \hline
%   \multirow{Data span $t_{span}[\mathrm{s}]$} & Number of successful identification & Success rate(\%) \\ \hline \hline
%     1.8 & 12 & 14.1 \\ \cline{1-3}
%     1.9 & 53 & 62.4 \\ \cline{1-3}
%     2.0 & 52 & 61.2 \\ \hline
%   \end{tabular}
% }
%   \label{identify snap process}
%   \end{center}
% \end{table}
% \end{center}
% \begin{center}
% \begin{table}[!h]
% \begin{center}
% \caption{Result of identification by search process}
% \scalebox{0.85}{  
% \begin{tabular}{|c|c|} \hline
%   \multirow{Number of successful identification} & Success rate(\%) \\ \hline \hline
%     47 & 55.3 \\ \hline
%   \end{tabular}
% }
%   \label{identify search process}
%   \end{center}
% \end{table}
% \end{center}
% \begin{center}
% \begin{table}[!h]
% \begin{center}
% \caption{Result of identification by both snap and search processes}
% \scalebox{0.85}{  
% \begin{tabular}{|c|c|c|c|c|} \hline
%   \multirow{Data span} & Improved identification & Deteriorated identification & Number of  & Success \\
%                 $t_{span}[\mathrm{s}]$ & by search process & by search process & successful identification & rate(\%) \\ \hline \hline
%     1.8 & 31 & 1 & 42 & 49.4 \\ \cline{1-5}
%     1.9 & 3 & 4 & 52 & 61.2 \\ \cline{1-5}
%     2.0 & 4 & 5 & 51 & 60.0 \\ \hline
%   \end{tabular}
% }
%   \label{identify both processes}
%   \end{center}
% \end{table}
% \end{center}
% \begin{center}
% \begin{table}[!h]
% \begin{center}
% \caption{Result of identification for each successful/failure pattern when $t_{span}=2.0[\mathrm{s}]$}
% \scalebox{0.85}{  
% \begin{tabular}{|c|c|c|c|c|c|} \hline
%   \multirow{Successful/failure} & Translational & Rotational & Success rate & Success rate & Success rate\\
%                 pattern & offset[{\mathrm{mm}}] & offset[$^\circ$] & by snap  & by search & by both\\
%                 (ground truth) &  &  & process(\%) & process(\%) &  processes(\%)\\ \hline \hline
%     Pattern(1) & -0.5 & -0.5 & 100 & 40 & 100 \\ \cline{1-6}
%     Pattern(1) & -0.5 & 0.5 & 60 & 80 & 100 \\ \cline{1-6}
%     Pattern(1) & -0.5 & 0 & 80 & 80 & 80 \\ \cline{1-6}
%     Pattern(1) & 0.5 & -0.5 & 100 & 40 & 100\\ \cline{1-6}
%     Pattern(1) & 0.5 & 0.5 & 60 & 40 & 60 \\ \cline{1-6}
%     Pattern(1) & 0.5 & 0 & 100 & 60 & 100 \\ \cline{1-6}
%     Pattern(1) & 0 & -0.5 & 100 & 100 & 100 \\ \cline{1-6}
%     Pattern(1) & 0 & 0.5 & 80 & 40 & 80 \\ \cline{1-6}
%     Pattern(1) & 0 & 0 & 60 & 80 & 40 \\ \cline{1-6}
%     Pattern(2) & 2 & 0 & 40 & 0 & 20 \\ \cline{1-6}
%     Pattern(3) & -2 & 0 & 40 & 0 & 20 \\ \cline{1-6}
%     Pattern(4) & 0 & 2 & 20 & 40 & 20 \\ \cline{1-6}
%     Pattern(5) & 0 & -2 & 0 & 20 & 20 \\ \cline{1-6}
%     Pattern(6) & 1.5 & 1.5 & 20 & 80 & 20 \\ \cline{1-6}
%     Pattern(7) & 1.5 & -1.5 & 0 & 80 & 0 \\ \cline{1-6}
%     Pattern(8) & -1.5 & 1.5 & 100 & 100 & 100 \\ \cline{1-6}
%     Pattern(9) & -1.5 & -1.5 & 80 & 60 & 60 \\ \hline
%   \end{tabular}
% }
%   \label{identify detail}
%   \end{center}
% \end{table}
% \end{center}
% 表\ref{identify snap process}より，スナップ工程での識別成功率は，
% データ区間$t_{span}[\mathrm{s}]=1.8$においては14.1\%，
% $t_{span}[\mathrm{s}]=1.9$においては62.4\%，
% $t_{span}[\mathrm{s}]=2.0$においては61.2$\%$であった．
% このことから，$t_{span}[\mathrm{s}]=1.8$\sim$1.9$の力情報が
% 作業部品間の物理作用を最も反映しており，成功パターンを識別するために重要であると考えられる．
% また，これら各区間は，スナップアセンブリが完了するよりも前の時点までの力情報であるため，提案手法による作業途中での成否パターンの識別可能性が示唆されたといえる．
% 特に，表\ref{identify detail}より，
% 成否パターン(1)の作業途中での識別精度は82.2\%と高く，スナップアセンブリの成功を迅速に検知可能である．
% 一方，表\ref{identify search process}，表\ref{identify both processes}より，
% 探り動作工程における識別精度はある程度高いことが確認されたにもかかわらず，
% 探り動作工程を導入した際の識別精度は改善されなかった．
% これについては，後述の考察で述べる．

\section{Error recovery}
\label{4.6}
% \ref{4.5}節で正しく識別されたいくつかのオフセットパターンに対して，\ref{3.5}節に従ってエラーリカバリシステムを構築した．
% 本実験では，以下のエラーリカバリ動作の生成パターンに該当するオフセットパターン(1)$\sim$(3)について，それぞれ3回ずつエラーリカバリ動作を行った．\\
% (1)成否パターン(1)において，エラーリカバリ動作を行わずに，ロボットハンドを下($+z$)方向に降ろすことで作業を完了させる場合($\Delta x= 0.5[{\mathrm{mm}}]$，$\Delta \theta_{z}=0.5[^\circ]$)\\
% (2)作業が失敗パターンである場合に，探り動作工程に移行することなくエラーリカバリ動作を生成する場合($\Delta x= 1.5[{\mathrm{mm}}]$，$\Delta \theta_{z}=-1.5[^\circ]$)\\
% (3)作業が失敗パターンである場合に，探り動作工程に移行し，探り動作工程での識別結果からエラーリカバリ動作を生成する場合($\Delta x= -1.5[{\mathrm{mm}}]$，$\Delta \theta_{z}=-1.5[^\circ]$)\\
% エラーリカバリを行った様子を
% 図\ref{recovery success}，
% \ref{recovery failure nosearch}，
% \ref{recovery failure search}
% に，エラーリカバリの成功率を表\ref{recovery table}に示す．
% ここで，エラーリカバリの成功率については，成否パターンの識別結果が成功パターン，失敗パターンいずれにおいても，識別後にスナップアセンブリが正しく完了された場合に成功したとする．
% \begin{figure}[p]
%     \begin{tabular}{c}
%       \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/recovery/recovery1_1.eps}
%           \hspace{1.6cm} (a) Snap process
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/recovery/recovery1_2.eps}
%           \hspace{1.6cm} (b) Finish snap assembly
%         \end{center}
%       \end{minipage}
%     \end{tabular}
%     \caption{Error recovery in offset pattern(1)}
%     \label{recovery success}
%   \end{figure}
% \begin{figure}[!h]
%     \begin{tabular}{c}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/recovery/recovery2_1.eps}
%           \hspace{1.6cm} (a) Snap process
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/recovery/recovery2_2.eps}
%           \hspace{1.6cm} (b) Error recovery motion
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/recovery/recovery2_3.eps}
%           \hspace{1.6cm} (c) Finish snap assembly
%         \end{center}
%       \end{minipage}
%     \end{tabular}
%     \caption{Error recovery in offset pattern(2)}
%     \label{recovery failure nosearch}
%   \end{figure}
% \begin{figure}[!h]
%     \begin{tabular}{c}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/recovery/recovery3_1.eps}
%           \hspace{1.6cm} (a) Snap process
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/recovery/recovery3_2.eps}
%           \hspace{1.6cm} (b) Right search process
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.33\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/recovery/recovery3_3.eps}
%           \hspace{1.6cm} (c) Left search process
%         \end{center}
%       \end{minipage}\\\\
%       \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=0.9\linewidth]{picture/chap4/recovery/recovery3_4.eps}
%           \hspace{1.6cm} (d) Error recovery motion
%         \end{center}
%       \end{minipage}
%       \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap4/recovery/recovery3_5.eps}
%           \hspace{1.6cm} (e) Finish snap assembly
%         \end{center}
%       \end{minipage}
%     \end{tabular}
%     \caption{Error recovery in offset pattern(3)}
%     \label{recovery failure search}
%   \end{figure}

\begin{center}
\begin{table}[htb]
\begin{center}
\caption{Result of error recovery}
  \begin{tabular}{|c|c|c|} \hline
  Offset pattern & Successful & Success rate \\ \hline \hline
  (1) & 3 & 100 \\ \cline{1-3}
  (2) & 3 & 100 \\ \cline{1-3}
  (3) & 3 & 100 \\ \hline
  \end{tabular}
  \label{recovery table}
\end{center}
\end{table}
\end{center}

% \begin{center}
% \begin{table}[h]
% \begin{center}
% \caption{Result of error recovery step}
% \scalebox{0.85}{  
% \begin{tabular}{|c|c|c|} \hline
%   \multirow{Offset pattern} & Successful & Success rate \\
%   & recovery & (\%)\\\hline \hline
%     (1) & 3 & 100 \\ \cline{1-3}
%     (2) & 3 & 100 \\ \cline{1-3}
%     (3) & 3 & 100 \\ \hline
%   \end{tabular}
% }
%   \label{recovery table}
%   \end{center}
% \end{table}
% \end{center}
% 表\ref{recovery table}より，
% 全てのエラーリカバリ行動において，部品を破損することなく
% スナップアセンブリを完了することができた．
% このことから，エラーリカバリシステムの有用性が示唆された．

\color{black}

==> section/06_discussion.tex <==
\section{discussion}
\label{sec:discussion}
%
%この章の内容は修論のデータから行ったものですので，今回の追加実験の結果とは別になります．
%


% 本章では，\ref{4}章の実験結果に対する考察を行い，提案手法の有用性を検討する．
% ここでは，
% 表\ref{node accuracy}$\sim$\ref{recovery table}
% にある結果に基づいて，
% スナップ工程のみでの識別結果，探り動作工程を導入した場合での識別結果それぞれについて，特に決定木の構築方法，及びその分類精度，また，作業途中での識別精度に対して評価を行う．
% その後，エラーリカバリの成功率について考察を行い，エラーリカバリシステム全体を評価する．

\subsection{Identification during assembly}
\label{5.1}
\subsubsection{Identification result by snap process}
\label{5.1.1}
% 成否パターン全体の識別精度については，
% \ref{4.5}節で述べた通り，表\ref{identify snap process}
% より，スナップ工程が完了するよりも前の時点までの力情報のみを用いて識別が達成されており，提案手法による作業途中での成否パターンの識別可能性が示唆されたといえる．
% ここで，本研究においては，スナップアセンブリ中のより早い段階で正しい識別が成されることは重要である．つまり，より少ないデータ区間を利用して上記が達成されることが望ましい．
% しかしながら，
% \ref{3.3_sec:feature_extraction}節を適用する波形データの区間について，より長い区間の波形データを用いた特徴量抽出であればあるほどより多くの波形情報を保持できるため，決定木の分類精度は向上する一方，未知データに対しては特徴量抽出の際，識別のために同等の長さの波形データ区間が必要となるため，作業途中での識別速度は低下すると考えられる．
% このことから，\ref{3.3_sec:feature_extraction}節を適用する波形データの区間の長さについて，決定木の分類精度と作業途中での識別速度にはトレードオフの関係があるといえる．
% 以上より，スナップアセンブリのより早い段階での識別を達成する問題は，
% 構築された決定木の分類精度が高く，かつそれを未知のスナップアセンブリに適用した際の識別速度が速くなるような波形データの区間を決定する問題に帰着される．
% 上記の問題を解決するには，
% 決定木の分類精度と利用データ区間を用いた評価式によって，特徴量抽出に最適なデータ区間を求める必要があるが，これについては今後の課題である．
%
% 次に，表\ref{identify detail}
% にある各成否パターンでの識別結果に基づいて評価を行う．\newline
% \begin{itemize}
% \item 成否パターン(1)について\newline
% これらは全て成否パターンの真値が(1)であるものであるが，82.2$\%$という高い識別成功率が得られた．実際に，成否パターン(1)を持つオフセットパターンが
% $\Delta x= 0[{\mathrm{mm}}]$，$\Delta \theta_{z}= 0.5[^\circ]$
% における波形データと成否パターン(2)を持つオフセットパターンが
% $\Delta x= 2[{\mathrm{mm}}]$，$\Delta \theta_{z}= 0[^\circ]$
% における波形データについて，
% 決定木図\ref{decision tree}
% のノード3にて識別に用いられた
% $x$軸まわりのトルクを比較したところ，図\ref{kousatsu s/fpattern1}
% のように顕著な相違性が確認された．
% このことからも，成否パターン(1)の作業途中での識別精度は高く，スナップアセンブリの成功を迅速に検知可能である．
% 一方，識別が失敗した検証データについて，成否パターン(9)であると誤識別した，オフセットパターンが
% $\Delta x= -0.5[{\mathrm{mm}}]$，$\Delta \theta_{z}=0[^\circ]$
% でのスナップアセンブリについては決定木図\ref{decision tree}
% より，ノード3にて
% 成否パターン(9)であると誤識別が発生していることがわかる．そこで，該当ノードにて識別に用いられた$y$軸方向にはたらく力の波形データについて，誤識別した波形データと，学習時に教師データを成否パターン(9)とした波形データを比較したところ，図\ref{kousatsu s/fpattern1_2}
% のように顕著な類似性が確認された．よって，検証時に取得された波形データが学習時と異なるものであり，異なる特徴量が抽出されたことが誤識別の原因であると考えられる．
% \begin{figure}[!h]
%   \begin{center}
%     \begin{tabular}{c}
% \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap5/waveform_sf1.eps}
%           \hspace{4cm} (a)Successful/failure pattern (1)
%         \end{center}
%       \end{minipage}
%      \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap5/waveform_sf2.eps}
%           \hspace{4cm} (b)Successful/failure pattern (2)
%         \end{center}
%       \end{minipage}\\\\
%     \end{tabular}
%     \caption{Torque data about $x$ axis corresponding to successful/failure patterns (1) and (2)}
%     \label{kousatsu s/fpattern1}
%   \end{center}
% \end{figure}
% \begin{figure}[!h]
%   \begin{center}
%     \begin{tabular}{c}
% \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap5/waveform_sf1_but_sf9.eps}
%           \hspace{4cm} (a)Successful/failure pattern (1)
%         \end{center}
%       \end{minipage}
%      \begin{minipage}{0.5\hsize}
%         \begin{center}
%           \includegraphics[width=\linewidth]{picture/chap5/waveform_sf9_learning.eps}
%           \hspace{4cm} (b)Successful/failure pattern (9)
%         \end{center}
%       \end{minipage}\\\\
%     \end{tabular}
%     \caption{Force data in $y$ axis corresponding to successful/failure patterns (1) obtained in validation step and (9) obtained in learning step}
%     \label{kousatsu s/fpattern1_2}
%   \end{center}
% \end{figure}
% 上記の問題は，作業部品やロボットハンドにパーツ等を取り付ける際のわずかな位置や角度の誤差によるものであると考えられ，実験環境を統一すれば提案手法は有効であると期待できる．
% \end{itemize}
% \begin{itemize}
% \item
% 成否パターン(3)について\newline
% 識別成功率は40\%であった．
% %探り動作工程を含めた場合ではパーセントであった．
% これについて，誤識別であった検証データについては全て成否パターン(8)と識別していたことから，構築された決定木図\ref{decision tree}のノード2において，成否パターン(3)と成否パターン(8)の分類が困難であることが考えられる．
% 実際にノード2(図\ref{classifier}(b))を確認したところ，成否パターン(3)である特徴量の多くが分離境界付近に位置しており，誤識別が発生しやすい状態であることが分かった．
% これについて，該当ノードにおいて，SVMを実行する力・トルク成分を$x$軸まわりのトルクに変更したところ，図\ref{changing_SVM_node}が得られた．またこれをノード2の代わりに新たなノードとした場合，成否パターン(3)の検証用データ全てにおいて，正しい識別が達成された．
% \begin{figure}[t]
%   \begin{center}
%           \includegraphics[width=0.75\linewidth]{picture/chap5/changed_node.eps}
%           %\includegraphics[width=\linewidth]{picture/chap1/test.eps}
%           \caption{Result of SVM when the selected force/torque parameter is torque about x-axis in node2 of decision tree in figure\ref{decision tree}}
%           \label{changing_SVM_node}
%         \end{center}
% \end{figure}
% 以上のことから，決定木の構築段階において，SVMを実行する力・トルク成分の選択方法に改善の余地が存在すると考えられる．
% 上記の解決策としては，SVMの実行結果に対する分類精度の計算方法について，式\ref{accuracy}ではなく，分類境界の持つ分類スコアの勾配情報がより反映されたものにすることが考えられる．
% 式\ref{accuracy}では，図\ref{classifier}(b)のように特徴量が分類境界付近に位置する場合において，識別時に誤識別に陥りやすい状態であるにかかわらず，
% 表\ref{node accuracy}に示すように高い分類精度が計算される．
% 一方，図\ref{changing_SVM_node}においては，一部の特徴量の誤分類は存在するものの，その他の特徴量については分類スコアが高く，全体的な分類精度は図\ref{classifier}(b)よりも高いといえる．
% 表\ref{node accuracy}において，各ノードで高い分類精度が得られているにもかかわらず
% 識別精度が同程度の比例をしていないのは上記の理由であるためであると考えられる．
% よって，分類精度式\ref{accuracy}を変更することで，決定木のノードの作成時に図\ref{classifier}(b)ではなく，より理想的な分類境界を持つ図\ref{changing_SVM_node}が選択されるため，識別精度の向上が期待できる．
% \end{itemize}

% \begin{itemize}
% \item 成否パターン(5)について\newline
% 識別成功率は0$\%$となり識別成功率が低かった．
% 誤識別であった検証データについては5つ中4つが成否パターン(6)と識別していたことから，
% 決定木図\ref{decision tree}においてノード8までは正しく識別されるが，ノード8において
% 成否パターン(5)と成否パターン(6)の識別が困難であることが考えられる．
% 実際，識別の際に参照されたノード8(図\ref{classifier}(h))を確認したところ，大部分の特徴量が成否パターン(6)と分類されており，成否パターン(5)と分類することが困難となっていることが分かった．
% またその他のデータ区間においても，SVMの実行時に同様の現象が確認できた．
% これは，成否パターンが(5)である学習データが成否パターン(6)であるものと比べて不足しており，SVMの実行時に対象データ間に偏りが生じたためであり，
% 成否パターン(2)，(3)，(4)においても同様の原因が識別成功率の低下に寄与していることが確認された．
% よって，学習データの少ない成否パターンに当たるオフセットパターンを増やして学習を行うことで解決されると考えられる．
%\end{itemize}

\subsubsection{Identification result by both snap and search processes}
\label{5.1.2}
% 次に，探り動作工程を導入した場合の識別成功率について考察を行う．
% 本実験では，成否パターン全体の識別精度については，
% 表\ref{identify both processes}
% より，データ区間$t_{span}[\mathrm{s}]=1.8$においては49.4$\%$，$t_{span}[\mathrm{s}]=1.9$においては61.2$\%$，$t_{span}[\mathrm{s}]=2.0$においては60.0$\%$であり，データ区間$t_{span}[\mathrm{s}]=1.8$の場合のみ識別精度が向上したが，それ以外のデータ区間では，わずかに識別精度が低下した．

% まず，
% データ区間$t_{span}[\mathrm{s}]=1.8$において識別精度が大きく向上したが，
% これは多くの識別において，スナップ工程での識別結果が棄却され，探り動作工程に識別を委ねられたためである．
% 表\ref{node accuracy}から分かるように，データ区間$t_{span}[\mathrm{s}]=1.8$では，該当区間までの力情報のみでは成否パターンを反映した特徴量を抽出することが困難であり，SVMの実行時に適切な分離境界が得られない．
% この場合，多くのオフセットパターンにおいてノードの持つ分類精度値は閾値以下であり，探り動作工程に移行することで表\ref{identify search process}
% にあるような識別精度が反映されたと考えられる．
% よって，探り動作工程を導入すれば，スナップ工程でのロボットハンドの降下時間を削減，
% つまり，移動量を減らした場合でも正しい識別が可能であり，より作業部品が破損しないアセンブリ工程を実現できると考えられる．一方，常に探り動作工程を必要とするため，探り動作工程によって作業部品が破損しないような配慮を行う必要があることや，
% 全体の作業時間が常に長くなる等の課題が存在するが，これらについては今後の課題である．

% 次に，データ区間$t_{span}[\mathrm{s}]=1.9$，$t_{span}[\mathrm{s}]=2.0$での識別結果について考察する．
% 本実験では，上記のデータ区間においては，
% %スナップ工程のみでの識別精度が60\%程度であるにもかかわらず，探り動作工程に移行する場合が少なく，探り動作工程による識別精度の向上が十分に表れなかった．
% 表\ref{identify detail}の成否パターン(4)，(5)，(6)，(7)にあるように，
% 探り動作工程の方がスナップ工程よりも良い識別精度であった成否パターンが確認されたが，
% 実際に探り動作工程に移行されることがわずかであった．
% さらに，探り動作工程に移行した場合においても
% 表\ref{identify both processes}にあるように，
% スナップ工程での識別結果が正しいものであるにもかかわらず，識別時に経由した決定木中のノードの持つ分類スコアが\ref{4.1}節で設定した閾値に満たなかったため，スナップ工程での識別が棄却されて探り動作工程での誤った識別を最終的な識別結果とした場合があり，
% 逆効果となってしまった識別も見られた．
% 以上より，\ref{3.5}節にある探り動作工程への移行必要性の判定基準に改善の余地があると考えられる．
% 提案手法では，経由ノードにおける分類スコアとノード自体の分類精度値に対して，
% それぞれ独立に評価して探り動作工程の必要性を判定していたが，\ref{5.2}節で考察したように，
% 例えば図\ref{classifier}(h)のような分離境界の場合，分類精度は低いにもかかわらず，分類スコアの絶対値が低い領域が限定されているため，探り動作工程へ移行しにくい．
% この場合，分類スコアの参照のみでは探り動作工程の必要性について適切な判定が困難である．
% 同様に，探り動作工程での識別結果を取得する際，
% 左探り動作工程と右探り動作工程で異なる識別結果であった場合に，適切な識別を選択しない場合もみられた．
% これらについては，改善された分類精度式\ref{accuracy}と
% 未知データから抽出される特徴量が決定木上で保持する分類スコアを組み合わせて
% より適切な判定式を提案することで解決されると考えられるが，これについては今後の課題である．

% また，表\ref{identify search process}の探り動作工程における識別成功率から，探り動作工程の内容自体についても改善の余地があると考えれる．
% 本実験結果では，全成否パターンに対しての識別成功率は55.3\%であった．
% 提案手法では，探り動作工程はロボットハンドを左右に数ミリ往復させる動作として統一していたが，上述の通り，左右の探り動作工程における識別結果が異なる場合や，ともに誤識別である場合が存在する．
% よって，スナップ工程から得られた情報から，より効率的な探り動作工程の内容を適応的に変化させることで，意義のある力情報が取得でき，識別精度を向上させることができると考えられる．
% 提案手法の場合，スナップ工程での決定木において，経由したノードの内，識別結果が信頼できるノードまでをスナップ工程での識別結果とし，可能性の残っている成否パターンに効果的な探り動作工程内容を選択することが考えられる．

\subsection{Error recovery}
\label{5.2}
% 次に，エラーリカバリの成功率について考察を行う．
% 本実験で行ったエラーリカバリ実験においては，
% 表\ref{recovery table}から，3種類のオフセットパターン(1)$\sim$(3)全てにおいてエラーリカバリが成功した．よって，エラーリカバリシステムの有用性が示唆された．
% しかし，エラーリカバリ行動の成功率は成否パターンの識別成功率に依存しているため，
% 上記の識別精度の向上がエラーリカバリシステム全体の精度を向上させるうえで重要である．
% また提案手法では，発生しているオフセットを解消する方向への移動量を一定値としていたが，この場合，大きなオフセットが発生している場合においては
% エラーリカバリ行動が不十分であり，再度作業の失敗が検知される恐れがある．
% これについては，成否パターンのみではなく，オフセットの量も識別する手法が必要であるが，これについては今後の課題である．

